Qr-Hint: Actionable Hints Towards Correcting Wrong SQL Queries

We describe a system called Qr-Hint that, given a (correct) target query Q* and a (wrong) working query Q, both expressed in SQL, provides actionable hints for the user to fix the working query so that it becomes semantically equivalent to the target. It is particularly useful in an educational setting, where novices can receive help from Qr-Hint without requiring extensive personal tutoring. Since there are many different ways to write a correct query, we do not want to base our hints completely on how Q* is written; instead, starting with the user's own working query, Qr-Hint purposefully guides the user through a sequence of steps that provably lead to a correct query, which will be equivalent to Q* but may still "look" quite different from it. Ideally, we would like Qr-Hint's hints to lead to the "smallest" possible corrections to Q. However, optimality is not always achievable in this case due to some foundational hurdles such as the undecidability of SQL query equivalence and the complexity of logic minimization. Nonetheless, by carefully decomposing and formulating the problems and developing principled solutions, we are able to provide provably correct and locally optimal hints through Qr-Hint. We show the effectiveness of Qr-Hint through quality and performance experiments as well as a user study in an educational setting.

==> examples/disjoint-tree/ex.tex <==


% ========================== Example ===========================

\begin{Example}\label{ex:disjoint-tree}
% Consider the following SQL logical formulae $P_1$ and $P_2$ where $P_1$ is the reference formula, and $a,b,c,d,e$ are integers. The syntax trees are shown in Figure ~\ref{fig:disjoint-tree}:

% \begin{itemize}
%     \item[] $P_1$: $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7))$
%     \item[] $P_2$: $(a=c \land (d \neq e \lor d>f)) \lor (a=c \land (d>11 \land d<7))$
% \end{itemize}

Consider the syntax trees shown in \Cref{fig:disjoint-tree} for $P_1$ and $P_2$. 
%In the most ideal scenario, the number of repair sites is $2$. 
If the number of repair sites in $P_2$ is limited to at most 2, then the repair sites are $S = \{N_4, N_7 \}$, and corresponding fixes $F_S$ are $(a=b)$ and $(d>10 \lor d<7)$ respectively; replacing the sub-formulas at $N_4$ and $N_7$ with these fixes will make $P_2$ equivalent to $P_1$. 
%If we replace $a=c$ with $a=b$ and replace $(d>11 \land d<7)$ with $(d>10 \lor d<7)$, $P_2$ becomes equivalent to $P_1$. 
%can be rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7))$ which is exactly the same as $P_1$. 

When the number of allowed repair sites is $1$, the only possible set of repair site in $P_2$ is $N_1$, and the fix is replacing it with the entire logical formula corresponding to $P_1$. 
%since $N_1$ is the least common ancestor of $N_4$ and $N_7$. 
%As a result, a set of corresponding fixes is $F \equiv \{(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7)) \}$ where the only syntax tree in $F$ is $P_1$. 

When the number of sites is $3$, a set of repair sites in $P_2$ is $S = \{N_4, N_{10}, N_{11} \}$ and a set of corresponding fixes $F_S$ is 
%\equiv 
$(a=b)$, $(d>10 \lor d<7)$, and $(d>10 \lor d<7)$, which makes $P_2$ equivalent to $P_1$.
%After replacement, $P_2$ would be rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7) \land (d>10 \lor d<7))$ which is equivalent to $P_1$. 

When the number of sites is $4$, a set of repair sites in $P_2$ is $S = \{N_4, N_9, N_{10}, N_{11} \}$ and a set of corresponding fixes $F_S$ is  $(a=b)$, $(d>f)$, $(d>10 \lor d<7)$, $(d>10 \lor d<7)$. Here $N_9$ is redundant, i.e., our algorithm can return false negatives, which can be removed by post-processing from the proposed hints. Also note that fixes are always a sub-formula, so we do not change the $\land$ in $N_7$ with an $\lor$.
%After replacement, $P_2$ would be also rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7) \land (d>10 \lor d<7))$ which is equivalent to $P_1$. 
\end{Example}

\cut{
\blue{The predicate in a HAVING clause of $Q_2$ is treated similar to that in the WHERE clause....}
\sr{YIHAO/AMIR: PLEASE ADD SOMETHING ABOUT HAVING -- ARE MAX/COUNT ETC treated as a constant?}
}
% Reconsider the syntax trees are shown in \Cref{fig:disjoint-tree}. 
% In the most ideal scenario, the number of repair sites is $2$. A set of repair sites in $P_2$ (marked in red) is $S \equiv \{N_4, N_7 \}$, and corresponding fixes are $F \equiv \{a=b, d>10 \lor d<7 \}$. If we replace $a=c$ with $a=b$ and replace $d>11 \land d<7$ with $d>10 \lor d<7$, $P_2$ can be rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7))$ which is exactly the same as $P_1$. 

% When the number of allowed repair sites is $1$, the only possible set of repair sites in $P_2$ is $S \equiv \{N_1 \}$ since $N_1$ is the least common ancestor of $N_4$ and $N_7$. As a result, a set of corresponding fixes is $F \equiv \{(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7)) \}$ where the only syntax tree in $F$ is $P_1$. 

% When $n=3$, a set of repair sites in $P_2$ is $S \equiv \{N_4, N_{10}, N_{11} \}$ and a set of corresponding fixes is $F \equiv \{a=b, d>10 \lor d<7, d>10 \lor d<7 \}$. After replacement, $P_2$ would be rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7) \land (d>10 \lor d<7))$ which is equivalent to $P_1$. 

% When $n=4$, a set of repair sites in $P_2$ is $I \equiv \{N_4, N_9, N_{10}, N_{11} \}$ and a set of corresponding fixes is $F \equiv \{a=b, d>f, d>10 \lor d<7, d>10 \lor d<7 \}$. After replacement, $P_2$ would be also rewritten as $(a=b \land (d \neq e \lor d>f)) \lor (a=c \land (d>10 \lor d<7) \land (d>10 \lor d<7))$ which is equivalent to $P_1$. 




